MPI Windows on Storage for HPC Applications

Upcoming HPC clusters will feature hybrid memories and storage devices per compute node. In this work, we propose to use the MPI one-sided communication model and MPI windows as unique interface for programming memory and storage. We describe the design and implementation of MPI storage windows, and present its benefits for out-of-core execution, parallel I/O and fault-tolerance. In addition, we explore the integration of heterogeneous window allocations, where memory and storage share a unified virtual address space. When performing large, irregular memory operations, we verify that MPI windows on local storage incurs a 55% performance penalty on average. When using a Lustre parallel file system, asymmetric performance is observed with over 90% degradation in writing operations. Nonetheless, experimental results of a Distributed Hash Table, the HACC I/O kernel mini-application, and a novel MapReduce implementation based on the use of MPI one-sided communication, indicate that the overall penalty of MPI windows on storage can be negligible in most cases in real-world applications.

==> Makefile <==

all: main.pdf

main.pdf: main.tex
	@pdflatex main.tex -interaction nonstopmode 2>&1 1>main.pdf.log
	@- bibtex main.aux 2>&1 1>main.pdf.log
	@pdflatex main.tex -interaction nonstopmode 2>&1 1>main.pdf.log
	@pdflatex main.tex -interaction nonstopmode 2>&1 1>main.pdf.log
	@while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log 2> /dev/null) do pdflatex main.tex -interaction nonstopmode 2>&1 1>main.pdf.log; done 2>&1 1>main.pdf.log

acmart.cls: acmart.ins
	latex acmart.ins

clean:
	@$(RM) *.log *.aux *.pdf \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

rebuild: clean all


